Scalable Motif Counting for Large-scale Temporal Graphs

One fundamental problem in temporal graph analysis is to count the occurrences of small connected subgraph patterns (i.e., motifs), which benefits a broad range of real-world applications, such as anomaly detection, structure prediction, and network representation learning. However, existing works focused on exacting temporal motif are not scalable to large-scale temporal graph data, due to their heavy computational costs or inherent inadequacy of parallelism. In this work, we propose a scalable parallel framework for exactly counting temporal motifs in large-scale temporal graphs. We first categorize the temporal motifs based on their distinct properties, and then design customized algorithms that offer efficient strategies to exactly count the motif instances of each category. Moreover, our compact data structures, namely triple and quadruple counters, enable our algorithms to directly identify the temporal motif instances of each category, according to edge information and the relationship between edges, therefore significantly improving the counting efficiency. Based on the proposed counting algorithms, we design a hierarchical parallel framework that features both inter- and intra-node parallel strategies, and fully leverages the multi-threading capacity of modern CPU to concurrently count all temporal motifs. Extensive experiments on sixteen real-world temporal graph datasets demonstrate the superiority and capability of our proposed framework for temporal motif counting, achieving up to 538* speedup compared to the state-of-the-art methods. The source code of our method is available at: https://github.com/steven-ccq/FAST-temporal-motif.

==> 07additional.tex <==

\clearpage
%  \appendix

%  \subsection{Additional Experimental Results}

%  \textbf{Accuracy Evaluation}

%  The counts of motif instances of all 2-node and 3-node, 3-edge temporal motifs with $\delta=600s$ detected by our method and EX algorithm on other datasets are shown in Fig.~\ref{fig.instances2} and Fig.~\ref{fig.instances3}. 



%  \textbf{Scalable Evaluation} 

%  Running time in seconds of parallel algorithms \wrt. $\#threads$ on other datasets are shown in Fig.~\ref{fig.Parallel2}. 

\begin{figure*}[h]
    \centering
    \vspace{-0mm}
    \subfigure[Email-Eu]{
    \includegraphics[width=0.47\linewidth]{figures/heatmap_email_600.pdf}
    }
  \hspace{1mm}
    \subfigure[Act-mooc]{
    \includegraphics[width=0.47\linewidth]{figures/heatmap_actmooc_600.pdf}
    }\\
  \vspace{-0mm}
  \subfigure[Bitcoinotc]{
    \includegraphics[width=0.47\linewidth]{figures/heatmap_bitcoinotc_600.pdf}
    }
    \hspace{1mm}
    \subfigure[Bitcoinalpha]{
    \includegraphics[width=0.47\linewidth]{figures/heatmap_bitcoinalpha_600.pdf}
    }\\
    \vspace{-0mm}
    \subfigure[SMS-A]{
    \includegraphics[width=0.47\linewidth]{figures/heatmap_sms_600.pdf}
    }
    \hspace{1mm}
    \subfigure[FBWALL]{
    \includegraphics[width=0.47\linewidth]{figures/heatmap_facebookwall_600.pdf}
    }\\
    \vspace{-0mm}
    \caption{Counts of motif instances of all 2-node and 3-node, 3-edge $\delta$-temporal motifs with $\delta=600s$ (supplement-1).}
    \label{fig.instances2}
    \vspace{-0mm}
\end{figure*}



\begin{figure*}[h]
    \centering
    \vspace{-0mm}
    \subfigure[MathOverflow]{
    \includegraphics[width=0.47\linewidth]{figures/heatmap_mathoverflow_600.pdf}
    }
    \hspace{1mm}
    \subfigure[Askubuntu]{
    \includegraphics[width=0.47\linewidth]{figures/heatmap_askubuntu_600.pdf}
    }\\
    \subfigure[IA-online-ads]{
    \includegraphics[width=0.47\linewidth]{figures/heatmap_iaonline_600.pdf}
    }
   \hspace{1mm}
    \subfigure[Rec-MovieLens]{
    \includegraphics[width=0.47\linewidth]{figures/heatmap_recmovies_600.pdf}
    }\\
    \vspace{-0mm}
    \subfigure[Soc-bitcoin]{
     \includegraphics[width=0.47\linewidth]{figures/heatmap_bitcoin_600.pdf}
     }
    \subfigure[RedditComments]{
     \includegraphics[width=0.47\linewidth]{figures/heatmap_reddit_600.pdf}
    }
    \vspace{-0mm}
    \caption{Counts of motif instances of all 2-node and 3-node, 3-edge $\delta$-temporal motifs with $\delta=600s$ (supplement-2).}
    \label{fig.instances3}
    \vspace{-0mm}
\end{figure*}




\begin{figure*}[h]
    \centering
    \hspace{-6mm}
    \includegraphics[width=1.01\linewidth]{figures/parallel_4.pdf}
    \vspace{-0mm}
    \caption{Running time in seconds of parallel algorithms \wrt. $\#threads$ (supplement). }
    \label{fig.Parallel2}
    \vspace{-0mm}
\end{figure*}

==> coverletter.tex <==


\section*{Response to Reviewers}

Thank you for the valuable suggestions. We have carefully gone through each comment and provided detailed responses below. Accordingly, we thoroughly updated the manuscript. For simplicity, we use $\mathbf{R_iO_j}$ to denote the $j$-th improvement opportunity suggested by Reviewer $i$. 


\subsection{Response to Reviewer \#1} 
We thank the reviewer for the insightful questions and advice. We have revised the manuscript and responded to each comment as follows.


\underline{$\mathbf{R_1O_1}$}: (1) Is there a way to define these motifs more generally? (2) If the proposed system would work for different types of motifs. 
% The paper focuses on very specific motifs (2-node and 3-node, 3-edge temporal motifs). These are then divided into pre-defined categories and then the algorithms use specially designed counters like the Quadruple counter to count the motifs. Is there a way to define these motifs more generally by the user for different applications? Also, it is not clear to me if the proposed system would work for different types of motifs or is it specific to only these kinds.

\textbf{Response}:
(1) In Def. 2, we define the temporal motif following the literature. It allows users to specify the types of motifs to their interest. 
(2) Although the proposed algorithms in this paper are specially optimized for 2-node and 3-node, 3-edge temporal motifs (36 types in total), which are considered as the most common types of motifs~\cite{benson2016higher}, our framework that is natively parallel is general. It will be able to efficiently count the higher-order (more nodes) temporal motifs by expanding the number of center nodes and slightly adapting the structure of the counters. This will be the main focus of our future work.  

We have added the above discussion in the sections of problem definition and conclusion.  
% Will include the above discussion in the revision. 

\underline{$\mathbf{R_1O_2}$}: Explain ``we leverage the traversal of the third edge to realize the scan of the second edge, which significantly reduces the computation cost. '' 
% While explaining the FAST-STAR algorithm for counting all kinds of star and pair temporal motifs the authors mention “instead of traversing all edges between the first edge and the third edge for the choice of the second edge, we leverage the traversal of the third edge to realize the scan of the second edge, which significantly reduces the computation cost.” It is not clear to me what this means and how is it reducing the cost significantly. 

\textbf{Response}:
In FAST-Star algorithm, the motif that forms earlier will be counted earlier. Given a motif, the edge that arrives first (first edge) and the edge that arrives last (third edge) determine the time it forms and its duration. The second edge must fall into this time duration. FAST-Star thus leverages this property to significantly reduce the search space of the second edge.  

To search the second edge, a simple implementation is to traverse all the edges between first edge and third edge after the third edge is identified. But this is time consuming. 
To further optimize the search of the second edge, in the process of determining the third edge we use two HashMaps ($m_{in}$ and $m_{out}$) to simultaneously record the situation of all the second edge candidates. We thus no longer need to traverse all the edges between the first and the third edges. 

We have added the above explanation in the section (Sec.~\ref{sec.complexity}) that analyzes the complexity. 

\underline{$\mathbf{R_1O_3}$}: Why repeatedly count and finally divide by three? 
% In the FAST-Tri algorithm the authors mention that “ in order to avoid counting errors, we do not do any processing, but repeatedly count and finally divide by three. ” This seems rather ad-hoc and how can this reliably ensure correct counting and removal of all double counting errors.

\textbf{Response}:
FAST-Tri counts each triangle motif exactly three times. So dividing by three ensures correctness. %Will add proof in the revision. 
This is because each triangle temporal motif instance can form three different types of triangle temporal motifs \wrt. its three vertices, respectively. 
For example, edge sequence $\langle(v_a, v_c, 8s), (v_d, v_a, 9s), (v_c, v_d, 17s)\rangle$ in Fig.~\ref{fig.toyexample} forms an instance of triangle temporal motif $M_{25}$. When $v_a$ is selected as the center node, this instance can be identified as an instance recorded in $Tri[{\rm III},o,in,o]$. When $v_c$ is selected as the center node, this instance would be detected as an instance recorded in $Tri[{\rm II},in,o,in]$. When $v_d$ is selected as the center node, this instance is recognized as an instance recorded in $Tri[{\rm I},o,in,o]$. 
In fact, the counters $Tri[{\rm III},o,in,o]$, $Tri[{\rm II},in,o,in]$ and $Tri[{\rm I},o,in,o]$ are isomorphic (see Fig.~\ref{fig.TriangleIsomorphic}). Therefore, as shown in Fig.~\ref{fig.TriangleIsomorphic}, each triangle temporal motif can be identified as three distinct triangle types based on its three different vertices respectively. 
That is, each triangle temporal motif is counted exactly three times.

In this work, we target on a counting framework that is natively parallel. To achieve this, we have to avoid any dependency among different processes/threads, while eliminating the repeated counting will inevitably introduce dependency. 
Therefore, repeatedly counting and dividing by three is an efficient solution. 

We have added the above discussion in Sec.~\ref{sec.tri-complexity} in the revised manuscript. 

\underline{$\mathbf{R_1O_4}$}: Does the proposed Hierarchical parallel framework (HARE) rely on OpenMP to handle load imbalance? 
% It is not clear in the paper how exactly does the proposed Hierarchical parallel framework (HARE) used to accelerate the counting of temporal motifs handle load imbalance. The authors mention that in the Inter-Node parallel mode the system relies on the the dynamic scheduling mode provided by OpenMP. While the Intra-node parallel mode relies on the reduction tool provided by OpenMP to copy the variables within node, so that each thread keeps the backup of these variables. Since this is a claimed contribution in the paper a little more detail and emphasis on novelty would be helpful.

\textbf{Response}: 
In our proposed hierarchical parallel framework (HARE), we propose two parallel strategies: inter-node and intra-node parallel mechanisms. 
% Since our proposed \model has inherent parallelism within and among nodes, 
Both modes use the tools provided by OpenMP. 
However, it is worth noting that it is the natively parallel nature of HARE that makes it possible to directly use OpenMP tools to handle load imbalance.

We have added the above discussion in Sec.~\ref{sec.parallel}.
% Will revise our draft to reflect the above discussion.  

% Following your suggestion, we will add more explanations for this contribution. 
% Although our proposed FAST naturally has high parallelism, simply employing multi-threading do not achieve the desired effect. This is because the degree distribution of the nodes in most temporal graphs is extremely unbalanced, which leads to the load imbalance problem of multi-threading.   To address this issue, we first propose the inter-node parallel mechanism, which is implemented by the dynamic scheduling mode provided by OpenMP to solve the problem of load imbalance at the node level.   
% However, we also find tat the few nodes with higher degrees (e.g., top ten nodes) account for the dominant part of the time consumption of whole graph. Therefore, the inter-node parallel mechanism cannot solve this kind of imbalance problem. 
% To this end, we further propose the intra-node parallel mechanism. Since the temporal motif counting process inside the node in our FAST also has high parallelism, the intra-node parallel can be implemented easily by the reduction tool provided by OpenMP.  




\underline{$\mathbf{R_1O_5}$}: How is the threshold for switching between the different parallel modes decided?

\textbf{Response}:
Given a dataset, if the degree of a node is higher than a threshold, we will enable the intra-node parallel mode. Otherwise, only the inter-node parallel mode will be enabled.

Through our experiment study, the degree distribution of most datasets follows a long-tailed distribution. We found that setting the threshold to the minimal degree of the top 20 nodes with the largest degrees works well on all datasets we tested in the experiments, indicating that setting this parameter is not hard.  


\underline{$\mathbf{R_1O_6}$}: (1) most of the datasets used in the experiments are small; (2) the accuracy of the counting is provided only on 4 datasets; (3) the comparison is done against only one baseline. 

\textbf{Response}:
(1) Per your suggestion, we perform new experiments on two larger temporal graphs with more than 100M  edges (\ie, Soc-bitcoin and RedditComments), where RedditComments contains more than 600M temporal edges. The new experimental results are reported in Table~\ref{tab.single_thread} and Fig.~\ref{fig.Parallel} in Sec.~\ref{sec.efficiency} and Sec.~\ref{sec.scale}. 
% \lei{Report the results here!!!} 

Specifically, in a single-threaded environment (see Table~\ref{tab.single_thread}), our \model improves $4.3\times$ and $7.8\times$ efficiency against EX algorithm on large-scale RedditComments and Soc-bitcoin datasets. 
In a multi-threaded environment (see Fig.~\ref{fig.Parallel}), our parallel framework \framework achieves $24\times$ and $21\times$ speedup on RedditComments and Soc-bitcoin as the number of threads increases from 1 to 32. In particular, \framework achieves $203\times$ and $97\times$ speedup against EX algorithm when $\#threads = 32$ on RedditComments and Soc-bitcoin datasets, respectively. 

Notice that in our current experiments, we have already used all large-scale temporal/dynamic graphs that are made publicly available by~\cite{snapnets,nr}.  



(2) We have the accuracy results on all datasets. But due to limited space, we only present the results on four datasets representing different degree distributions and different scales. 
The experimental results on other datasets can be found in Fig. 13 and Fig. 14 in the online document at~\textcolor{red}{\url{https://github.com/steven-ccq/FAST-temporal-motif/blob/main/appendix.pdf}}. 
% Will put all results in an extended version and make it accessible to reviewers. 

(3) We compare against EX~\cite{paranjape2017motifs} published in WSDM 2017. To the best of our knowledge, it is still the state-of-the-art method that exactly counts temporal motifs in temporal graphs. 


\underline{$\mathbf{R_1O_7}$}: Explain why the results shown in Table III have a huge variability in the speedup performance across different datasets. 
% Table III shows the speedup of the proposed technique while using a single thread across different datasets. There is a huge variability of speedup performance across the different datasets that is observed. Please explain the reason for this variability.

\textbf{Response}:
As discussed in the time complexity analysis, our two algorithms both achieve a time complexity linear to the number of temporal edges of the input graph. However, the time complexity also correlates to the average degree $d^{\delta}$ of nodes within time interval $\delta$, which is different on different datasets. On the other hand, the performance of the baselines (\eg, EX) also relies on the characteristics of the datasets (\eg, the number of induced triangles). Both lead to the variability of the speedup across different datasets. 

We have added the above explanation in Sec.~\ref{sec.efficiency} in this revision. 

\subsection{Response to Reviewer \#2} 
We thank the reviewer for the valuable questions and advice. 


\underline{$\mathbf{R_2O_1}$}: Introduce the counting of triangle motifs in more detail. 
% This paper proposes a hierarchical parallel framework. In terms of the triangle motif, deciding the first and third edge could extract the information, but the second edge is based on other nodes. It is better to explain such issues and introduce more details about this framework.

\textbf{Response}:
Per your suggestion, we expand the discussion on triangle temporal motif (Sec.~\ref{sec.triangle}) in the revision. 

To identify potential triangle motifs, we first choose a node in graph $\mathcal{G}$ as the center node $u$, and then determine two different temporal edges connected to center node $u$ such that the other two connected nodes are different. We denote these two temporal edges as $e_i=(t_i,v,dir_i)$ and $e_j=(t_j,w,dir_j)$, where $t_j- t_i \leq \delta$, and $dir_i$ and $dir_j$ are the directions of $e_i$ and $e_j$ \wrt. center node $u$, respectively.  
Each edge between $v$ and $w$ and the two edges above may form triangle temporal motifs, depending on whether the time constraint $\delta$ is satisfied. 
Therefore, we next consider each edge $e_k$ between nodes $v$ and $w$ that satisfies the time constrain $\delta$. Let $t_k$ be the timestamp of edge $e_k$ and $dir_k$ be the direction of edge $e_k$ \wrt. node $v$ (\ie, $o$ indicates from $v$ to $w$ and $in$ denotes from $w$ to $v$). Unlike FAST-Star, the order of the three edges is determined by their timestamps. 
Then according to the order of three edges, we determine the types of potential triangle temporal motif and use corresponding counter to count the triangle temporal motif. 

% In triangle motif, we first determine two different edges connected to center node u such that the other two connected nodes (denoted by v and w) are different. Each edge between v and w and the two edges above may potentially form motifs, depending on whether the time constraint $\delta$ is satisfied.  Unlike FAST-Star, the order of three edges is determined by the timestamps on three edges. 

\underline{$\mathbf{R_2O_2}$}: In Algorithm 1, how to initialize the two HashMaps?
% In Algorithm 1, this paper utilizes two HashMap to record the related information. As these structures are used from beginning of method, how to initializing them is important. However, this paper lacks the introduction about this part. 

\textbf{Response}:
% Algorithm 1 always initializes the two HaspMaps to empty at the beginning of each iteration.  Will discuss this process in more detail. 
Following your suggestion, we add more explanation in the revision.

In Algorithm~\ref{alg.FastStar}, in the process of determining the third edge, we use two HashMaps (\ie, $m_{in}$ and $m_{out}$) to simultaneously record the direction and the number of all the second edge candidates. We thus no longer need to traverse all the edges again between the first and the third edges. 
Therefore, $m_{in}$ and $m_{out}$ are always initialized to be empty at the beginning of each iteration. 


\underline{$\mathbf{R_2O_3}$}: New Exp.: (1) Larger datasets should be tested; (2) Justify the applications mentioned in Section 1. 
% The experimental evaluation could be further improved: (1) Larger datasets should be tested; (2) It would be better to justify the applications mentioned in Section 1 by performing some experiments.

\textbf{Response}:
(1) Per your suggestion, we run additional experiments on two new larger temporal graphs with more than 100M edges (\ie, Soc-bitcoin and RedditComments), where RedditComments contains more than 600M temporal edges. 
The new experimental results are updated in Table~\ref{tab.single_thread} and Fig.~\ref{fig.Parallel}. 
Please see Sec.~\ref{sec.efficiency} and Sec.~\ref{sec.scale} for details.  
% \lei{again, report the results here!!!}

Notice that in our current experiments, we have already used all large-scale temporal/dynamic graphs that are made publicly available by~\cite{snapnets,nr}. 

(2) Several works~\cite{liu2021motif,huang2020motif,yu2019rum} have justified that incorporating motifs into network embedding improves the quality of the learned representations, while clearly the efficiency of motif detection methods is critical to scale network embedding to big data.  
% Due to limited space, we did not perform similar experiments again. 



\subsection{Response to Reviewer \#3} 
We thank the reviewer for the constructive questions and advice. 

\underline{$\mathbf{R_3O_1}$}: Explain why the speedup of HARE versus HARE-Pair for different datasets is very different. 

\textbf{Response}:
As suggested, we explain this phenomenon in the revision. 
Notice that we use dual ordinate axes in Fig.~\ref{fig.Parallel}. HARE and EX refer to left ordinate axis, while HARE-Pair and BTS-Pair refer to right ordinate axis. Since HARE and HARE-Pair refer to different axes (different scales), their relative positions in the figures are not comparable. 

\underline{$\mathbf{R_3O_2}$}: Verify if the dynamic scheduling OpenMP indeed solved the problem of load imbalance by comparing against a diagram that does not use dynamic scheduling. 
% It is mentioned that the dynamic scheduling mode provided by OpenMP solved the problem of load imbalance, so this claim should be verified in a new diagram where runtimes are compared before and after using the dynamic scheduling. 

\textbf{Response}: 
Thank you for the insightful suggestion. In Sec.~\ref{sec.parameter}, we have verified the effectiveness of the dynamic scheduling model of OpenMP on WikiTalk dataset. In Fig.~\ref{fig.sensitivity}(b), `dynamic' denotes that dynamic scheduling model of OpenMP is used, and `without $thr_d$' means that default (static) scheduling mode is used. 
As shown in Fig.~\ref{fig.sensitivity}(b), dynamic scheduling indeed significantly outperforms the version without it (\ie, dynamic vs. without $thr_d$).  

We have explained this in Sec.~\ref{sec.parameter} in the revision.  

\underline{$\mathbf{R_3O_3}$}: What tools the baseline methods are using for parallel speedup. 
% It is mentioned that the proposed algorithm is using OpenMP for achieving parallel speedup while it is not clarified what tools (if any) the baseline methods are using for parallel speedup.  

\textbf{Response}: 
As suggested, we add the description for this in the section of experimental setting (Sec.~\ref{sec.setting}) in the revision. 

To run in parallel, all baselines use the same OpenMP mode to our method for parallel speedup. 


==> tables/Triangle_Isomorphic.tex <==
\begin{table}[]
\begin{center}
\renewcommand\arraystretch{1.5}
\caption{There are 24 instances of the counter $Tri[Type,dir_i,dir_j,dir_k]$, but only 8 non-isomorphic triangle motifs}
\label{triangle_isomorphic}
\setlength{\tabcolsep}{2mm}{}
\begin{tabular}{|c|c|}
\hline
Isomorphic                                & Motifs    \\ \hline
Tri(I,i,o,o) Tri(II,i,i,0) Tri(III,o,o,i) & $M_{35}$ \\ \hline
Tri(I,o,o,o) Tri(II,i,i,i) Tri(III,o,i,i) & $M_{45}$ \\ \hline
Tri(I,i,i,o) Tri(II,i,o,o) Tri(III,o,o,o) & $M_{16}$ \\ \hline
Tri(I,o,i,o) Tri(II,i,o,i) Tri(III,o,i,o) & $M_{25}$ \\ \hline
Tri(I,i,o,i) Tri(II,o,i,o) Tri(III,i,o,i) & $M_{26}$ \\ \hline
Tri(I,o,o,i) Tri(II,o,i,i) Tri(III,i,i,i) & $M_{46}$ \\ \hline
Tri(I,i,i,i) Tri(II,o,o,o) Tri(III,i,o,o) & $M_{16}$ \\ \hline
Tri(I,o,i,i) Tri(II,o,o,i) Tri(III,i,i,o) & $M_{36}$ \\ \hline
\end{tabular}
\end{center}
\end{table}

==> tables/ablation_study.tex <==
\begin{table}[]
\begin{center}
\caption{Ablation experiment results.}
\label{tale.ablation_experiments_results} % Comparison of variations.
\setlength{\tabcolsep}{1mm}{}

\begin{tabular}{c|cccccc}
\toprule
 Dataset & \multicolumn{3}{c}{Hangzhou City}& \multicolumn{3}{c}{Jinan City}\\ 
 Methods & $MAPE_t$& $MAPE_p$ & $RMSE$ & $MAPE_t$& $MAPE_p$ & $RMSE$\\ 
\midrule

\modelta  &0.3078  &0.4483  &34.6892   & 0.4431	&0.4259  &33.0753\\
\modelpe  &0.2888  &0.4197  & 31.5093  &0.4728  &0.5052  &35.8841  \\
\modelrw  & 0.3286 & 0.5055  & 34.1412  &0.4434   & 0.4256 & 33.0653 \\
\modelvl  & 0.3957  & 0.4683  & 38.0991  & 0.4814  & 0.4936 &36.0105 \\
\modelc   & 0.3480  &  0.4136  & 34.3503 &0.4389   &0.4275  &33.4542    \\
\modelr   & 0.3086 & 0.3946   & 32.4999  &0.4463   &0.4280  &33.1873   \\ 
\modeld   & $\backslash$   &$\backslash$  & $\backslash$  &0.4412  &0.4281  &33.1672   \\ 
\modelw   & $\backslash$   & $\backslash$ & $\backslash$  & 0.4451  & 0.4298  &33.2166 \\ 
\midrule
\model       & 0.2420 & 0.3368 &28.8727 &0.3884  &0.3780  &30.2166  \\

\bottomrule
\end{tabular}
\end{center}
\vspace{-5mm}
\end{table}

==> tables/tune_hyperparameter.tex <==
\begin{table}[]
\begin{center}
\caption{Comparison of different hyperparameters.}
\label{tune_hyperparameters}
\setlength{\tabcolsep}{1mm}{}
\begin{tabular}{c|cccccc}
\toprule
 Dataset & \multicolumn{3}{c}{Hangzhou City}& \multicolumn{3}{c}{Jinan City}\\ 
 Methods & $MAPE_t$& $MAPE_p$ & $RMSE$ & $MAPE_t$& $MAPE_p$ & $RMSE$\\ 
\midrule
$\mathcal{L}_{-walk}$   & 0.3286 & 0.5055  & 34.1412  &0.4700   & 0.4256 & 33.0653 \\
$\mathcal{L}_{-volume}$ & 0.3957  & 0.4683  & 38.0991  & 0.4504  & 0.4632 &32.0465 \\
$\mathcal{L}_{-current}$ & 0.3480  &  0.4136  & 34.3503 &0.4742   &0.4275  &33.4542    \\
$\mathcal{L}_{-recent}$  & 0.3086 & 0.3946   & 32.4999  &0.4731   &0.4280  &33.1873   \\ 
$\mathcal{L}_{-daily}$   & $\backslash$   &$\backslash$  & $\backslash$  &0.4738  &0.4281  &33.1672   \\ 
$\mathcal{L}_{-weekly}$   & $\backslash$   & $\backslash$ & $\backslash$  &0.4717  &0.4298  &33.2166   \\ 
% $\mathcal{L}_{joint}$ & 0.2420 & 0.3368 &28.8727 &0.3892  &0.4875  &45.0415  \\
$\mathcal{L}_{joint}$ & 0.2420 & 0.3368 &28.8727 &0.3884  &0.3780  &30.2166  \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-2mm}
\end{table}
